Measuring Nuclear Matter Parameters with NICER and LIGO/Virgo

The NICER Collaboration recently reported the measurement of the mass and radius of a pulsar PSR J0030+0451. We here use this new measurement to constrain one of the higher-order nuclear matter parameters $K_{\mathrm{sym,0}}$. We further combine the tidal measurement of the binary neutron star merger GW170817 by LIGO/Virgo to derive a joint 1-$\sigma$ constraint as $K_{\mathrm{sym,0}} = -102^{+71}_{-72}$ MeV. We believe this is the most reliable bound on the parameter to date under the assumption that there is no new physics above the saturation density which impacts neutron star observations.

==> NICER-GW (3)/preamble.tex <==
\usepackage{mathtools}
\usepackage{physics}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{dcolumn}
\usepackage{bm}
\usepackage{dsfont} 
\usepackage{amsmath,amssymb}
\usepackage{hyperref}
\usepackage{tabularx}
\usepackage{epsf,epsfig}
\usepackage[normalem]{ulem}
\usepackage[usenames]{color}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{diagbox}
\usepackage[abs]{overpic}
\allowdisplaybreaks
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=blue,
    citecolor=blue
}
\urlstyle{same}

\usepackage{pagecolor}
\usepackage{bm}


\newcommand{\red}[1]{\protect\color{red} #1 \protect\color{black}}
\newcommand{\green}[1]{\protect\color{green} #1 \protect\color{black}}
\newcommand{\blue}[1]{\protect\color{blue} #1 \protect\color{black}}
\newcommand{\black}[1]{\protect\color{black} #1 \protect\color{black}}
\newcommand{\yellow}[1]{\protect\color{yellow} #1 \protect\color{black}}
%\newcommand{\bra}[1]{\protect\langle #1 |}
%\newcommand{\ket}[1]{| #1 \protect\rangle}
%\newcommand{\braket}[2]{\protect\langle #1 | #2 \protect\rangle}
%\newcommand{\expected}[1]{\protect\langle #1 \protect\rangle}
\newcommand{\R}{{\mbox{\tiny R}}}
\newcommand{\M}{{\mbox{\tiny M}}}
\newcommand{\ky}[1]{\textcolor{cyan}{\it{\textbf{ky: #1}}} }
\newcommand{\kent}[1]{\textcolor{magenta}{\textbf{ #1}} }
\newcommand{\zack}[1]{\textcolor{magenta}{\textbf{#1}}}
\newcommand{\zc}[1]{\textcolor{blue}{\it{\textbf{zc: #1}}} }
\newcommand{\jz}[1]{\textcolor{orange}{\it{\textbf{jz: #1}}}}
\newcommand{\josef}[1]{\textcolor{magenta}{\textbf{#1}}}
\definecolor{red(ncs)}{rgb}{0.77, 0.01, 0.2}
\definecolor{utk}{rgb}{1.0, 0.51, 0.0}
\newcommand{\ny}[1]{\textcolor{blue}{NY: #1} }
\newcommand{\kc}[1]{\textcolor{green}{KC: #1} }
\newcommand{\ch}[1]{\textcolor{red}{CH: #1} }
\newcommand{\aws}[1]{\textcolor{utk}{#1} }
\newcommand{\chs}[1]{\textcolor{red}{\sout{ #1} } }
\newcommand{\NS}{{\mbox{\tiny NS}}}
\newcommand{\sci}[2]{{#1 \times 10^{#2}}}
\newcommand{\msol}{M_{\odot}}
\newcommand{\mev}{\mathrm{MeV}}
\newcommand{\sym}{\mathrm{sym,0}}

%\newcommand{\ksympm}[3]{K_\sym = {#1}^{+{#2}}_{-{#3}}~\mev}

\usepackage{array}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}


\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}

\def\eq#1{Eq.~(\ref{eq:#1})}
\def\Eq#1{Equation~(\ref{eq:#1})}
\def\eqs#1#2{Eqs.~(\ref{eq:#1}) \& (\ref{eq:#2})}
\def\eqlist#1#2{Eqs.~(\ref{eq:#1}-\ref{eq:#2})}
\def\Eqs#1#2{Equations~(\ref{eq:#1}) \& (\ref{eq:#2})}
\def\Eqlist#1#2{Equations~(\ref{eq:#1}-\ref{eq:#2})}
\def\fig#1{Fig.\ref{fig:#1}}
\def\figs#1#2{Figs.\ref{fig:#1} \& \ref{fig:#2}}
\def\Fig#1{Figure~\ref{fig:#1}}
\def\Figs#1#2{Figures~\ref{fig:#1} \& \ref{fig:#2}}
\def\tab#1{Table~\ref{tab:#1}}
\def\sec#1{Section~\ref{sec:#1}}


